A posteriori error estimates for finite element discretizations of time-harmonic Maxwell's equations coupled with a non-local hydrodynamic Drude model

We consider finite element discretizations of Maxwell's equations coupled with a non-local hydrodynamic Drude model that accurately accounts for electron motions in metallic nanostructures. Specifically, we focus on a posteriori error estimation and mesh adaptivity, which is of particular interest since the electromagnetic field usually exhibits strongly localized features near the interface between metals and their surrounding media. We propose a novel residual-based error estimator that is shown to be reliable and efficient. We also present a set of numerical examples where the estimator drives a mesh adaptive process. These examples highlight the quality of the proposed estimator, and the potential computational savings offered by mesh adaptivity.

==> figures/bowtie/curve_s080.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/bowtie/s080/curve.txt} node [pos=.6,pin=-90:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/bowtie/s080/curve.txt} node [pos=.95,pin=90:{$\eta/\omega$}] {};

\plot[domain=1.5e3:8e4] {5e3*x^(-1.)};
\SlopeTriangle{.1}{-.15}{.25}{-1.}{$N_{\rm dofs}^{-1}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the bowtie example
with $\omega = 0.8\omegaP$.}
\label{fig_cv_bowtie_s080}
\end{figure}


==> figures/bowtie/curve_s090.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/bowtie/s090/curve.txt} node [pos=.6,pin=-90:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/bowtie/s090/curve.txt} node [pos=.95,pin=90:{$\eta/\omega$}] {};

\plot[domain=1.5e3:3e5] {.5e4*x^(-1.)};
\SlopeTriangle{.1}{-.15}{.25}{-1.}{$N_{\rm dofs}^{-1}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the bowtie example
with $\omega = 0.9\omegaP$.}
\label{fig_cv_bowtie_s090}
\end{figure}


==> figures/bowtie/curve_s100.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/bowtie/s100/curve.txt} node [pos=.15,pin=135:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/bowtie/s100/curve.txt} node [pos=.95,pin=90:{$\eta/\omega$}] {};

\plot[domain=1.5e3:1e6] {1e3*x^(-1.)};
\SlopeTriangle{.1}{-.15}{.25}{-1.}{$N_{\rm dofs}^{-1}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the bowtie example
with $\omega = \omegaP$.}
\label{fig_cv_bowtie_s100}
\end{figure}


==> figures/bowtie/sol_s080.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s080/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s080/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the bowtie experiment with $\omega = 0.8\omegaP$}
\label{figure_bowtie_sol_s080}
\end{figure}


==> figures/bowtie/sol_s090.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s090/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s090/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the bowtie experiment with $\omega = 0.9\omegaP$}
\label{figure_bowtie_sol_s090}
\end{figure}


==> figures/bowtie/sol_s100.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s100/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/bowtie/s100/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the bowtie experiment with $\omega = \omegaP$}
\label{figure_bowtie_sol_s100}
\end{figure}


==> figures/groove/sol_s080.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s080/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s080/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = 0.8\omegaP$}
\label{figure_groove_sol_s080}
\end{figure}


==> figures/groove/sol_s090.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s090/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s090/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = 0.9\omegaP$}
\label{figure_groove_sol_s090}
\end{figure}


==> figures/groove/sol_s100.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s100/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/groove/s100/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = \omegaP$}
\label{figure_groove_sol_s100}
\end{figure}


==> figures/triangle/curve_s070.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/triangle/s070/curve.txt} node [pos=.6,pin=-90:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/triangle/s070/curve.txt} node [pos=.95,pin=90:{$\eta/\omega$}] {};

\plot[domain=3.e3:1e5] {1e4*x^(-3./2.)};

\SlopeTriangle{.1}{-.15}{.25}{-3./2.}{$N_{\rm dofs}^{-3/2}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the nanotip example
with $\omega = 0.7\omegaP$.}
\label{fig_cv_nanotip_s070}
\end{figure}


==> figures/triangle/curve_s100.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/triangle/s100/curve.txt} node [pos=.7,pin=-90:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/triangle/s100/curve.txt} node [pos=.95,pin=90:{$\eta/\omega$}] {};

\plot[domain=3.e3:9e4] {8e4*x^(-3./2.)};

\SlopeTriangle{.1}{-.15}{.25}{-3./2.}{$N_{\rm dofs}^{-3/2}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the nanotip example
with $\omega = \omegaP$.}

\label{fig_cv_nanotip_s100}

\end{figure}


==> figures/triangle/curve_s130.tex <==
\begin{figure}

\begin{tikzpicture}
\begin{axis}
[
	xlabel = {$N_{\rm dofs}$},
	ylabel = {Errors scaled by $\omega$},
	xmode  = log,
	ymode  = log
]

\addplot[color=blue,mark=o     ] table [x = nr_dofs, y = true_error]%
{figures/triangle/s130/curve.txt} node [pos=.8,pin=-90:{$\xi/\omega$}] {};

\addplot[color=red ,mark=square] table [x = nr_dofs, y = esti_error]%
{figures/triangle/s130/curve.txt} node [pos=.9,pin=90:{$\eta/\omega$}] {};

\plot[domain=3.e3:3e5] {5e4*x^(-3./2.)};

\SlopeTriangle{.1}{-.15}{.3}{-3./2.}{$N_{\rm dofs}^{-3/2}$}{}

\end{axis}
\end{tikzpicture}

\caption{Convergence history of the adaptive algorithm for the nanotip example
with $\omega = 1.3\omegaP$.}

\label{fig_cv_nanotip_s130}

\end{figure}


==> figures/triangle/error_level_s070.tex <==
\begin{figure}

\includegraphics[width=\linewidth]{figures/triangle/s070/true_err_24.pdf}

\includegraphics[width=\linewidth]{figures/triangle/s070/esti_err_24.pdf}

\caption{Actual (top panel) and estimated (bottom panel) errors at the iteration
\#25 of the adaptive algorithm for the nanotip example with $\omega = 0.7\omegaP$.}
\label{fig_el_nanotip_s070}
\end{figure}


==> figures/triangle/error_level_s100.tex <==
\begin{figure}

\includegraphics[width=\linewidth]{figures/triangle/s100/true_err_24.pdf}

\includegraphics[width=\linewidth]{figures/triangle/s100/esti_err_24.pdf}

\caption{Actual (top panel) and estimated (bottom panel) errors at the iteration
\#25 of the adaptive algorithm for the nanotip example with $\omega = \omegaP$.}
\label{fig_el_nanotip_s100}
\end{figure}


==> figures/triangle/mesh_s070.tex <==
\begin{figure}

\begin{minipage}{.35\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s070/mesh_49.pdf}
\end{minipage}
\begin{minipage}{.60\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s070/mesh_49_crop.pdf}
\end{minipage}

\caption{Computational mesh at the \#50 iteration of the adaptive algorithm for
the nanotip example with $\omega = 0.7\omegaP$. The right panel presents a focus
on the inclusion.}
\label{fig_fm_nanotip_s070}
\end{figure}


==> figures/triangle/mesh_s100.tex <==
\begin{figure}

\begin{minipage}{.35\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s100/mesh_49.pdf}
\end{minipage}
\begin{minipage}{.60\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s100/mesh_49_crop.pdf}
\end{minipage}

\caption{Computational mesh at the \#50 iteration of the adaptive algorithm for
the nanotip example with $\omega = \omegaP$. The right panel presents a focus
on the inclusion.}
\label{fig_fm_nanotip_s100}
\end{figure}


==> figures/triangle/sol_s070.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s070/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s070/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = 0.7\omegaP$}
\label{figure_triangle_sol_s070}
\end{figure}


==> figures/triangle/sol_s100.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s100/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s100/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = \omegaP$}
\label{figure_triangle_sol_s100}
\end{figure}


==> figures/triangle/sol_s130.tex <==
\begin{figure}

\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s130/E_norm}
\end{minipage}
\begin{minipage}{.45\linewidth}
\includegraphics[width=\linewidth]{figures/triangle/s130/J_norm}
\end{minipage}

\hspace{.5cm} $|\BE|$ \hspace{6.5cm} $|\BJ|$

\caption{Field intensities in the nanotip experiment with $\omega = 1.3\omegaP$}
\label{figure_triangle_sol_s130}
\end{figure}

